Equivariant Sheaf Neural Networks: Learning Geometric Transport on Graphs

Equivariant graph neural networks provide a principled way to model geometric systems, but efficient first-order architectures remain limited in how vector information can be transformed as it moves across a graph. We introduce \textsc{ESNN}, an Equivariant Sheaf Neural Network that enriches this interaction by learning directed, matrix-valued transport between neighboring vector features while preserving exact Euclidean equivariance. Rather than increasing the order of the representation, ESNN keeps scalar and vector features first-order and places the additional geometric flexibility in the edge transport itself. We characterize this transport theoretically, showing that when relative displacement is the only covariant geometric input, every linear $O(n)$-equivariant map decomposes into independent radial and tangential components, while learned covariant features enable richer feature-conditioned transformations. We also introduce controlled symmetry relaxation for systems with a preferred ambient direction, which may be prescribed or inferred from data while recovering full $E(n)$-equivariance when the directional pathway is inactive. Across particle dynamics, mesh-based simulation, point-cloud classification, and molecular property prediction, ESNN improves dynamics prediction, recovers the gravity axis when symmetry is broken, yields substantial gains on selected mesh tasks and long-horizon rollouts, and remains robust to unseen rotations. These results show that learning how geometric information is transported across edges offers a complementary route to expressive equivariant message passing without requiring higher-order representations.

==> img/esnn_visual_abstract.tex <==
% ESNN main teaser figure body (revised TikZ vector figure, v2).
% Requires: \usepackage{tikz,amsmath,amssymb,xcolor}
% \usetikzlibrary{arrows.meta,calc,positioning}

\begin{tikzpicture}[
  x=1cm,y=1cm,>=Latex,
  font=\sffamily,
  panel/.style={rounded corners=6pt, draw=#1!75!black, line width=.9pt, fill=#1!2},
  box/.style={rounded corners=3.5pt, draw=#1!55!black, line width=.6pt, fill=#1!6},
  atom/.style={circle, ball color=gray!35, draw=black!45, minimum size=4.0mm, inner sep=0pt},
  nodeball/.style={circle, fill=gray!15, draw=black!70, minimum size=6.3mm, inner sep=0pt, font=\normalsize\itshape},
  mini/.style={circle, fill=gray!15, draw=black!65, minimum size=4.5mm, inner sep=0pt, font=\scriptsize\itshape},
  bond/.style={draw=black!58, line width=1.0pt},
  arr/.style={-Latex, line width=1.05pt},
  redarr/.style={arr, draw=red!80!black},
  bluearr/.style={arr, draw=blue!75!black},
  greenarr/.style={arr, draw=green!50!black},
  purplearr/.style={arr, draw=violet!75!black},
  grayline/.style={draw=black!14, line width=.6pt},
  title/.style={font=\sffamily\bfseries\Huge, align=center},
  subtitle/.style={font=\sffamily\large, text=black!72, align=center},
  ptitle/.style={font=\sffamily\bfseries\LARGE, align=center},
  label/.style={font=\sffamily\normalsize, align=center},
  smalllabel/.style={font=\sffamily\footnotesize, align=center},
  tinylabel/.style={font=\sffamily\scriptsize, align=center},
]

\definecolor{eqred}{RGB}{190,32,28}
\definecolor{sheaforange}{RGB}{207,126,13}
\definecolor{esnngreen}{RGB}{20,120,50}
\definecolor{esnnblue}{RGB}{24,82,190}
\definecolor{softblue}{RGB}{236,245,255}
\definecolor{softred}{RGB}{255,242,242}
\definecolor{softorange}{RGB}{255,248,235}
\definecolor{softgreen}{RGB}{240,252,242}

% ------------------------------------------------------------------
% Helper commands
% ------------------------------------------------------------------
\newcommand{\numdot}[3]{\node[circle, fill=#2, text=white, font=\bfseries\large, minimum size=8.2mm, inner sep=0pt] at (#1) {#3};}
\newcommand{\good}[2]{\node[font=\bfseries\Large, text=green!55!black] at (#1,#2) {$\checkmark$};}
\newcommand{\bad}[2]{\node[font=\bfseries\Large, text=red!75!black] at (#1,#2) {$\times$};}
\newcommand{\pair}[3]{\node[nodeball] (#1i) at (#2,#3) {$i$};\node[nodeball] (#1j) at ($(#1i)+(1.75,0)$) {$j$};\draw[bond] (#1i)--(#1j);}
\newcommand{\molecule}[3]{%
\begin{scope}[shift={(#1,#2)}, scale=#3]
  \coordinate (a) at (-.95,0); \coordinate (b) at (-.4,.68); \coordinate (c) at (.35,.62); \coordinate (d) at (.92,.02); \coordinate (e) at (.36,-.64); \coordinate (f) at (-.45,-.58);
  \draw[bond] (a)--(b)--(c)--(d)--(e)--(f)--(a); \draw[bond] (b)--(e);
  \foreach \p in {a,b,c,d,e,f}{\node[atom] at (\p) {};}
\end{scope}}
\newcommand{\moleculeB}[3]{%
\begin{scope}[shift={(#1,#2)}, scale=#3, rotate=-16]
  \coordinate (a) at (-1.02,.02); \coordinate (b) at (-.35,.84); \coordinate (c) at (.48,.55); \coordinate (d) at (1.05,-.25); \coordinate (e) at (.26,-.82); \coordinate (f) at (-.67,-.48);
  \draw[bond] (a)--(b)--(c)--(d)--(e)--(f)--(a); \draw[bond] (b)--(e);
  \foreach \p in {a,b,c,d,e,f}{\node[atom] at (\p) {};}
\end{scope}}
\newcommand{\gridpatch}[3]{%
\begin{scope}[shift={(#1,#2)}, scale=#3]
  \draw[fill=blue!8, draw=blue!50, line width=.55pt] (0,0)--(1.35,.28)--(1.35,1.08)--(0,.80)--cycle;
  \foreach \t in {.2,.4,.6,.8}{\draw[blue!35] ($(0,0)!\t!(1.35,.28)$)--($(0,.8)!\t!(1.35,1.08)$);}
  \foreach \t in {.2,.4,.6,.8}{\draw[blue!35] ($(0,0)!\t!(0,.8)$)--($(1.35,.28)!\t!(1.35,1.08)$);}
\end{scope}}
\newcommand{\vortex}[3]{%
\begin{scope}[shift={(#1,#2)}, scale=#3]
  \foreach \r/\a in {.18/20,.33/55,.49/90,.66/125,.82/160}{\draw[blue!65, line width=.5pt, -Latex] (\a:\r) arc[start angle=\a,end angle=\a+220,radius=\r];}
\end{scope}}

% ------------------------------------------------------------------
% Canvas
% ------------------------------------------------------------------


% Panel geometry
\def\ybot{2.95}\def\pH{9.95}\def\pW{7.70}
\coordinate (A) at (.35,\ybot);
\coordinate (B) at (8.65,\ybot);
\coordinate (C) at (16.95,\ybot);

% ------------------------------------------------------------------
% Panel A
% ------------------------------------------------------------------
\draw[panel=eqred] (A) rectangle ++(\pW,\pH);
\numdot{.90,12.40}{black}{1}
\node[ptitle, text=eqred!78!black, anchor=west] at (1.42,12.40) {Equivariant GNNs};
\node[label, text=black!65] at (4.20,11.95) {symmetry-preserving, but mostly radial};

\molecule{1.85}{11.00}{.64}
\draw[arr, line width=1.15pt] (3.45,11.00)--(4.25,11.00);
\moleculeB{5.95}{11.00}{.64}
\draw[redarr, line width=1.1pt] (1.22,10.55)--(1.96,11.25);
\draw[redarr, line width=1.1pt] (5.55,10.55)--(6.25,11.25);
\node[label, text=eqred!85!black] at (4.20,10.12) {radial / distance-based interactions};
\draw[grayline] (.72,9.83)--(7.70,9.83);

% compression row
\node[anchor=west, font=\bfseries\normalsize] at (.90,9.35) {compression};
\pair{aComp}{2.70}{9.15}
\draw[redarr] ($(aCompi)+(-.68,.10)$)--($(aCompi)+(-.22,.10)$);
\draw[redarr] ($(aCompj)+(.68,.10)$)--($(aCompj)+(.22,.10)$);
\node[smalllabel, text=green!45!black, anchor=west] at (5.35,9.15) {captured};
\good{7.22}{9.15}
\draw[grayline] (.72,8.62)--(7.70,8.62);

% shear row
\node[anchor=west, font=\bfseries\normalsize] at (.90,8.14) {shear};
\pair{aShear}{2.70}{7.94}
\draw[bluearr, dashed] ($(aSheari)+(0,.34)$)--++(0,.72);
\draw[bluearr, dashed] ($(aShearj)+(0,-.34)$)--++(0,-.72);
\node[smalllabel, text=red!75!black, anchor=west] at (5.35,7.94) {missed};
\bad{7.22}{7.94}
\draw[grayline] (.72,7.41)--(7.70,7.41);

% torsion row
\node[anchor=west, font=\bfseries\normalsize] at (.90,6.93) {torsion};
\pair{aTor}{2.70}{6.73}
\draw[purplearr, dashed] ($(aTori)+(-.12,.32)$) arc[start angle=140,end angle=392,radius=.34];
\draw[purplearr, dashed] ($(aTorj)+(-.12,.32)$) arc[start angle=140,end angle=392,radius=.34];
\node[smalllabel, text=red!75!black, anchor=west] at (5.35,6.73) {missed};
\bad{7.22}{6.73}
\draw[grayline] (.72,6.20)--(7.70,6.20);

% anisotropy row
\node[anchor=west, font=\bfseries\normalsize] at (.90,5.72) {anisotropy};
\node[mini] (ani) at (3.35,5.52) {$i$};
\foreach \ang in {25,70,115,205,250,295}{\draw[arr, draw=black!75, line width=.7pt] (ani)--++(\ang:.58);}
\node[smalllabel, text=red!75!black, anchor=west] at (5.35,5.52) {collapsed};
\bad{7.22}{5.52}

\node[box=eqred, text=eqred!78!black, font=\bfseries\normalsize, minimum width=6.9cm, minimum height=.92cm] at (4.18,4.05) {Equivariant, but spatially isotropic};
\node[label, text=black!60, text width=6.8cm] at (4.18,3.32) {cannot independently route transverse or torsional modes};

% ------------------------------------------------------------------
% Panel B
% ------------------------------------------------------------------
\draw[panel=sheaforange] (B) rectangle ++(\pW,\pH);
\numdot{8.98,12.40}{black}{2}
\node[ptitle, text=sheaforange!90!black, anchor=west] at (9.50,12.40) {Standard SheafNNs};
\node[label, text=black!65] at (12.30,11.95) {direction-aware, but unconstrained};

\pair{bTop}{9.95}{10.80}
\foreach \dy/\col in {.30/red!80!black,.10/green!55!black,-.10/blue!75!black,-.30/violet!78!black}{\draw[arr, draw=\col, line width=1pt] ($(bTopi)+(.42,\dy)$)--($(bTopj)+(-.42,\dy)$);}
\begin{scope}[shift={(12.60,10.62)}, rotate=18]
  \draw[fill=sheaforange!18, draw=sheaforange!75!black] (-.50,-.40) rectangle (.50,.40);
  \foreach \x in {-.25,0,.25}{\draw[sheaforange!55] (\x,-.40)--(\x,.40);}
  \foreach \y in {-.20,0,.20}{\draw[sheaforange!55] (-.50,\y)--(.50,\y);}
\end{scope}
\node[label, text=sheaforange!85!black] at (12.35,10.00) {rich learned edge transports};
\draw[grayline] (9.02,9.72)--(16.02,9.72);

\node[anchor=west, font=\bfseries\normalsize] at (9.10,9.18) {Rotation/reflection test};
\node[label, text=black!60] at (12.38,8.76) {does the message rotate with the system?};
\node[nodeball] (b0i) at (9.75,7.72) {$i$}; \node[nodeball] (b0j) at (10.98,7.72) {$j$}; \draw[bond] (b0i)--(b0j);
\foreach \dy/\col in {.26/red!80!black,.08/green!55!black,-.10/blue!75!black,-.28/violet!78!black}{\draw[arr, draw=\col, line width=.95pt] ($(b0i)+(.34,\dy)$)--($(b0j)+(-.32,\dy)$);}
\draw[-Latex, line width=1.0pt, draw=black!65] (11.55,7.86)..controls(12.25,8.55)and(13.05,8.55)..(13.75,7.86);
\node[font=\normalsize] at (12.65,8.42) {$Q$};
\node[nodeball] (b1i) at (14.15,7.40) {$i'$}; \node[nodeball] (b1j) at (15.25,7.96) {$j'$}; \draw[bond] (b1i)--(b1j);
\foreach \dy/\col in {.26/red!80!black,.08/green!55!black,-.10/blue!75!black,-.28/violet!78!black}{\draw[arr, draw=\col, line width=.95pt] ($(b1i)+(.26,\dy)$)--($(b1j)+(-.22,\dy)$);}
\draw[red!75!black, dashed, -Latex, line width=.9pt] (10.95,7.10)..controls(12.05,6.20)and(13.30,6.20)..(14.45,7.00);
\node[font=\bfseries\LARGE, text=red!75!black] at (12.72,6.55) {$!$};
\node[label, text=red!75!black, font=\normalsize\bfseries, text width=6.1cm] at (12.38,5.90) {transport does not transform consistently};

\node[box=sheaforange, text=red!70!black, font=\bfseries\normalsize, minimum width=6.9cm, minimum height=.92cm] at (12.48,4.05) {Anisotropic, but generally not equivariant};
\node[label, text=black!60, text width=6.8cm] at (12.48,3.32) {routing is expressive but not symmetry safe};

% ------------------------------------------------------------------
% Panel C
% ------------------------------------------------------------------
\draw[panel=esnngreen] (C) rectangle ++(\pW,\pH);
\numdot{17.28,12.40}{esnngreen!80!black}{3}
\node[ptitle, text=esnngreen!70!black, anchor=west] at (17.80,12.40) {Equivariant SheafNNs};
\node[label, text=black!65] at (20.85,11.95) {anisotropic and equivariant};

% ESNN: factorized transport
\molecule{18.10}{10.90}{.56}
\node[box=esnnblue, minimum width=.85cm, minimum height=.70cm, text=esnnblue, font=\bfseries\Large] (sblock) at (19.95,11.15) {$S$};
\node[box=esnngreen, minimum width=.85cm, minimum height=.70cm, text=esnngreen, font=\bfseries\Large] (tblock) at (19.95,10.35) {$T$};
\draw[arr, line width=1.15pt] (18.88,10.75)--(19.25,10.75);
\draw[bluearr, line width=1.05pt] (19.25,10.98)--(sblock.west);
\draw[greenarr, line width=1.05pt] (19.25,10.52)--(tblock.west);
\draw[arr, line width=1.15pt] (20.46,10.75)--(20.95,10.75);
\foreach \dy/\col in {.30/red!80!black,.10/green!55!black,-.10/blue!75!black,-.30/violet!78!black}{\draw[arr, draw=\col, line width=1pt] (20.94,10.75+\dy)--(22.20,10.75+\dy);}
\moleculeB{23.25}{10.88}{.56}
\node[smalllabel, text=esnnblue, text width=1.9cm] at (18.95,9.82) {geometry\\alignment};
\node[smalllabel, text=esnngreen!55!black, text width=1.9cm] at (21.55,9.82) {channel\\routing};
\node[label, text=black!65, text width=6.6cm] at (20.85,9.25) {separate spatial transport from feature mixing};
\draw[grayline] (17.32,8.95)--(24.30,8.95);

% Full physics row
\node[anchor=west, font=\bfseries\normalsize, text=esnngreen!60!black] at (17.42,8.45) {Full directional physics};
% compression
\begin{scope}[shift={(18.30,7.55)}]
\node[mini] (c1) at (0,0) {};
\node[mini] (c2) at (.95,0) {};
\draw[bond](c1)--(c2);
\draw[redarr](-.52,.10)--(-.12,.10);
\draw[redarr](1.47,.10)--(1.06,.10);
\node[smalllabel] at (.47,-.56) {compression};
\good{1.60}{.00}
\end{scope}
% shear
\begin{scope}[shift={(20.45,7.18)}]
\gridpatch{-.45}{-.10}{.70}
\draw[bluearr](-.75,.62)--(-.28,.96);
\draw[bluearr](1.20,-.08)--(.70,-.42);
\node[smalllabel] at (.28,-.64) {shear};
\good{1.66}{.26}
\end{scope}
% torsion
\begin{scope}[shift={(23.05,7.55)}]
\node[mini](tt1)at(-.70,0){};
\node[mini](tt2)at(0,0){};
\node[mini](tt3)at(.70,0){};
\draw[bond](tt1)--(tt2)--(tt3);
\draw[purplearr,dashed](-.88,.22)arc[start angle=150,end angle=400,radius=.32];
\draw[purplearr,dashed](.50,.22)arc[start angle=150,end angle=400,radius=.32];
\node[smalllabel] at (0,-.56) {torsion};
\good{1.20}{.00}
\end{scope}
\draw[grayline] (17.32,6.60)--(24.30,6.60);

% rotation consistency
\node[anchor=west, font=\bfseries\normalsize, text=esnngreen!60!black] at (17.42,6.15) {Rotation consistency};
\node[nodeball] (e0i) at (18.05,5.30) {$i$}; \node[nodeball] (e0j) at (19.15,5.30) {$j$}; \draw[bond](e0i)--(e0j);
\foreach \dy/\col in {.26/red!80!black,.08/green!55!black,-.10/blue!75!black,-.28/violet!78!black}{\draw[arr, draw=\col, line width=.95pt] ($(e0i)+(.34,\dy)$)--($(e0j)+(-.28,\dy)$);}
\draw[-Latex, line width=1.0pt, draw=black!65] (19.72,5.42)..controls(20.42,6.12)and(21.22,6.12)..(21.92,5.42);
\node[font=\normalsize] at (20.82,6.00) {$Q$};
\node[nodeball] (e1i) at (22.35,5.02) {$i'$}; \node[nodeball] (e1j) at (23.45,5.58) {$j'$}; \draw[bond](e1i)--(e1j);
\foreach \dy/\col in {.26/red!80!black,.08/green!55!black,-.10/blue!75!black,-.28/violet!78!black}{\draw[arr, draw=\col, line width=.95pt] ($(e1i)+(.26,\dy)$)--($(e1j)+(-.22,\dy)$);}
\good{24.00}{5.28}
\node[label, font=\normalsize\bfseries, text=green!48!black, text width=6.0cm] at (20.85,4.48) {rotated input $\Rightarrow$ rotated output};

\node[box=esnngreen, text=esnngreen!55!black, font=\bfseries\normalsize, minimum width=6.9cm, minimum height=.92cm] at (20.82,4.05) {Equivariant geometry $+$ anisotropic routing};
\node[label, text=black!60, text width=6.9cm] at (20.82,3.30) {geometry stays symmetry-correct; channels route directionally};

% ------------------------------------------------------------------
% Bottom strip
% ------------------------------------------------------------------
\draw[rounded corners=6pt, draw=black!20, fill=black!1] (.35,.78) rectangle (24.65,2.45);
\node[font=\bfseries\normalsize] at (12.50,2.17) {Why this matters: physical systems combine compression, shear, torsion, vorticity, and anisotropic environments};
\node[smalllabel, text width=2.5cm] at (2.25,1.58) {molecular\\conformations};
\molecule{3.95}{1.33}{.40}
\node[smalllabel, text width=2.2cm] at (6.95,1.58) {elastic\\deformation};
\gridpatch{7.95}{1.00}{.68}
\node[smalllabel, text width=2.0cm] at (11.00,1.58) {fluid\\vorticity};
\vortex{12.10}{1.35}{.50}
\draw[black!25] (13.45,1.02)--(13.45,2.0);
\node[font=\bfseries\normalsize, text=esnngreen!55!black] at (14.65,1.40) {ESNN};
\node[box=esnnblue, text=esnnblue, minimum width=2.45cm, minimum height=.65cm, font=\normalsize] at (16.65,1.40) {geometry};
\node[font=\Large] at (18.40,1.40) {$+$};
\node[box=esnngreen, text=esnngreen!55!black, minimum width=2.45cm, minimum height=.65cm, font=\normalsize] at (20.45,1.40) {routing};
\node[font=\Large] at (22.20,1.40) {$=$};
\node[font=\bfseries\normalsize, text=esnngreen!55!black] at (23.25,1.40) {both};

\draw[rounded corners=4pt, draw=esnnblue!65, fill=softblue, line width=.7pt] (2.70,-.82) rectangle (22.35,.12);
\node[font=\bfseries\normalsize, text=esnnblue] at (4.85,-.35) {Key insight:};
\node[font=\normalsize, text=black!75, anchor=west] at (6.30,-.35) {decouple \textit{geometric equivariance} from \textit{anisotropic topological routing}.};

\end{tikzpicture}


==> tables/ESNN_Architectures_Derivations.tex <==
\begin{table}[h]
\centering
\caption{\emph{Prevailing Equivariant Architectures as Constrained Special Cases of ESNN}. Each row identifies the algebraic constraint imposed on the transport matrices of Equation~4 and the resulting structural limitation.}
\label{tab:unification}
\smallskip
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Architecture} & \textbf{Spatial Connection} $\mathbf{S}_{ij}$ & \textbf{Topological Mixing} $\mathbf{T}_{ij}$ & \textbf{Tensor Product Integrity} & \textbf{Structural Limitation} \\
\midrule
EGNN~\citep{satorras2022enequivariantgraphneural}
    & $\mathbf{I}_n$
    & $\mathbf{I}_{c_v}$
    & Collapsed ($c_v = 0$)
    & Restricted to isotropic scalar distances. \\
\addlinespace
GVP~\citep{jing2020learning} / Vector Neurons~\citep{deng2021vector}
    & $\mathbf{I}_n$
    & Weight matrix $\mathbf{W}$
    & Preserved ($\mathbb{R}^n \otimes \mathbb{R}^{c_v}$)
    & Assumes globally aligned frames; blind to local gauge misalignment. \\
\addlinespace
PaiNN~\citep{schutt2021equivariant}
    & $\mathbf{P}_{\mathrm{rad}}$
    & Scalar gate $\mathrm{diag}(f_s)$
    & Preserved ($\mathbb{R}^n \otimes \mathbb{R}^{c_v}$)
    & Radial synthesis only; blind to transverse shear. \\
\addlinespace
GNN-LF~\citep{wang2022graph}
    & $\mathbf{Q}_i$
    & $\mathbf{I}_{c_v}$
    & Prematurely contracted
    & Collapses the covariant bundle into scalar invariants. \\
\addlinespace
PCA Frame Averaging~\citep{puny2022frame}
    & $\mathbf{Q}_i^{\top}\mathbf{Q}_j$
    & Weight matrix $\mathbf{W}$
    & Preserved ($\mathbb{R}^n \otimes \mathbb{R}^{c_v}$)
    & PCA frames degenerate on symmetric or coplanar motifs. \\
\addlinespace
Gauge CNNs~\citep{cohen2019gauge}
    & $\rho(\psi_{ij})$
    & Weight matrix $\mathbf{W}$
    & Preserved ($\mathbb{R}^n \otimes \mathbb{R}^{c_v}$)
    & Connection precomputed from a fixed mesh or manifold. \\
\addlinespace
Torsor CNNs~\citep{li2025learning}
    & $\rho(\psi_{ij})$
    & Weight matrix $\mathbf{W}$
    & Preserved ($\mathbb{R}^n \otimes \mathbb{R}^{c_v}$)
    & Edge potentials fixed by synchronization, not by node features. \\
\addlinespace
SE(3)-Transformer ($L{=}1$)~\citep{fuchs2020se}
    & $\mathbf{P}_{\mathrm{rad}},\, \mathbf{P}_{\mathrm{tan}}$
    & Attention $\alpha^{(k)}_{ij} \mathbf{I}_{c_v}$
    & Preserved ($\mathbb{R}^n \otimes \mathbb{R}^{c_v}$)
    & Isotropic attention; no channel-specific spatial routing. \\
\midrule
\textbf{ESNN (Ours)}
    & $\mathbf{P}_{\mathrm{rad}},\, \mathbf{P}_{\mathrm{tan}}$
    & Edge-gated $\mathbf{A}_{ij},\, \mathbf{B}_{ij}$
    & Preserved ($\mathbb{R}^n \otimes \mathbb{R}^{c_v}$)
    & \textit{Maximal class of linear $O(n)$-equivariant transports (Thm.~4.4)} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/QM9.tex <==
% \begin{table*}[t]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2.8pt}
% \renewcommand{\arraystretch}{0.95}

% \caption{
% \emph{QM9 Quantum-Chemistry Benchmark}.
% Mean absolute error (MAE) on twelve molecular properties.
% External baseline entries reproduce the current comparison and require source
% and data-partition verification under the final protocol. ESNN variants are
% shown in \textbf{bold}. A $\dagger$ denotes results obtained using different data partitions.
% Target units and the aggregate summary columns also require final definition.
% For every property, lower is better.
% }
% \label{tab:qm9_results}

% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lcccccccccccccc@{}}
% \toprule

% \textbf{Method}
% & $\boldsymbol{\alpha}$
% & $\boldsymbol{\Delta\epsilon}$
% & $\boldsymbol{\epsilon_{\mathrm{HOMO}}}$
% & $\boldsymbol{\epsilon_{\mathrm{LUMO}}}$
% & $\boldsymbol{\mu}$
% & $\boldsymbol{C_v}$
% & $\boldsymbol{G}$
% & $\boldsymbol{H}$
% & $\boldsymbol{\langle R^2\rangle}$
% & $\boldsymbol{U}$
% & $\boldsymbol{U_0}$
% & \textbf{ZPVE}
% & \textbf{std.}
% & \textbf{log} \\

% \midrule
% \multicolumn{15}{l}{\emph{Invariant models}} \\
% \midrule

% Cormorant
% & 85
% & 61
% & 34
% & 38
% & 38
% & 26
% & 20
% & 21
% & 961
% & 21
% & 22
% & 2.03
% & 2.14
% & -4.75 \\

% NMP
% & 92
% & 69
% & 43
% & 38
% & 30
% & 40
% & 19
% & 17
% & 180
% & 20
% & 20
% & 1.50
% & 1.78
% & -5.08 \\

% DimeNet++$\dagger$
% & 44
% & 32.6
% & 24.6
% & 19.5
% & 29.7
% & 23
% & 7.56
% & 6.53
% & 331
% & 6.28
% & 6.32
% & 1.21
% & 0.98
% & -5.67 \\

% ComENet$\dagger$
% & 45
% & 32.4
% & 23.1
% & 19.8
% & 24.5
% & 22
% & 7.98
% & 6.86
% & 259
% & 6.82
% & 6.69
% & 1.20
% & 0.93
% & -5.69 \\

% SphereNet$\dagger$
% & 46
% & 31.1
% & 22.8
% & 18.9
% & 24.5
% & 22
% & 7.78
% & 6.33
% & 268
% & 6.36
% & 6.26
% & 1.12
% & 0.91
% & -5.73 \\

% \midrule
% \multicolumn{15}{l}{\emph{Scalarization-based models}} \\
% \midrule

% ClofNet
% & 63
% & 53
% & 33
% & 25
% & 40
% & 27
% & 9
% & 9
% & 610
% & 9
% & 8
% & 1.23
% & 1.37
% & -5.37 \\

% EGNN
% & 71
% & 48
% & 29
% & 25
% & 29
% & 31
% & 12
% & 12
% & 106
% & 12
% & 11
% & 1.55
% & 1.23
% & -5.43 \\

% PaiNN$\dagger$
% & 45
% & 45.7
% & 27.6
% & 20.4
% & 12.0
% & 24
% & 7.35
% & 5.98
% & 66
% & 5.83
% & 5.85
% & 1.28
% & 1.01
% & -5.85 \\

% LEFTNet
% & 48
% & 40
% & 24
% & 18
% & 12
% & 23
% & 7
% & 6
% & 109
% & 7
% & 6
% & 1.33
% & 0.91
% & -5.82 \\

% EQGAT
% & 53
% & 32
% & 20
% & 16
% & 11
% & 24
% & 23
% & 24
% & 382
% & 25
% & 25
% & 2.00
% & 0.86
% & -5.28 \\

% ET
% & 59
% & 36.1
% & 20.3
% & 17.5
% & 11
% & 26
% & 7.62
% & 6.16
% & 33
% & 6.38
% & 6.15
% & 1.84
% & 0.84
% & -5.90 \\

% Geoformer
% & 40
% & 33.8
% & 18.4
% & 15.4
% & 10
% & 22
% & 6.13
% & 4.39
% & 28
% & 4.41
% & 4.43
% & 1.28
% & 0.75
% & -6.12 \\

% SaVeNet-B$\dagger$
% & 39
% & 24.8
% & 18.4
% & 16.3
% & 9.3
% & 23
% & 6.64
% & 5.43
% & 58
% & 5.48
% & 5.43
% & 1.18
% & 0.69
% & -6.04 \\

% \midrule
% \multicolumn{15}{l}{\emph{Equivariant Sheaf Neural Networks}} \\
% \midrule

% \textbf{ESNN-Id}
% & 63.08
% & 65.35
% & 43.13
% & 28.52
% & 58.81
% & 37.83
% & 15.76
% & 18.71
% & 749.44
% & --
% & 10.54
% & 1.54
% & --
% & -- \\

% \textbf{ESNN-Diag}
% & 62.16
% & 43.69
% & 27.44
% & 21.43
% & 17.15
% & 31.57
% & 11.48
% & 12.71
% & 134.99
% & 11.77
% & 13.57
% & 1.62
% & --
% & -- \\

% \textbf{ESNN-Ortho}
% & 79.42
% & 43.35
% & 25.10
% & 23.17
% & 21.77
% & 36.50
% & 17.76
% & 26.07
% & 323.52
% & 18.59
% & 25.25
% & 1.94
% & --
% & -- \\

% \textbf{ESNN-RadTan}
% & 60.32
% & 39.01
% & 25.16
% & 19.17
% & 16.08
% & 31.57
% & 14.77
% & 13.86
% & 119.11
% & 10.63
% & 10.34
% & 1.45
% & --
% & -- \\

% \bottomrule
% \end{tabular}%
% }
% \end{table*}



\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.8pt}
\renewcommand{\arraystretch}{0.95}

\caption{
\emph{QM9 molecular-property prediction.}
Mean absolute error (MAE) on twelve invariant molecular properties.
Baseline values and data-partition annotations follow the comparison reported
by \citet{aykent2025gotennet}. A $\dagger$ denotes results obtained using
different data partitions and should therefore not be interpreted as a strictly
matched comparison. Within the ESNN block, the best result for each property
is shown in \textbf{bold}. Target units follow the standard QM9 reporting
convention shown in the second header row. Lower is better.
}
\label{tab:qm9_results}

\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule

\textbf{Method}
& $\boldsymbol{\alpha}$
& $\boldsymbol{\Delta\epsilon}$
& $\boldsymbol{\epsilon_{\mathrm{HOMO}}}$
& $\boldsymbol{\epsilon_{\mathrm{LUMO}}}$
& $\boldsymbol{\mu}$
& $\boldsymbol{C_v}$
& $\boldsymbol{G}$
& $\boldsymbol{H}$
& $\boldsymbol{\langle R^2\rangle}$
& $\boldsymbol{U}$
& $\boldsymbol{U_0}$
& \textbf{ZPVE} \\

\textbf{Units}
& $\mathrm{m}a_0^3$
& meV
& meV
& meV
& mD
& $\mathrm{mcal\,mol^{-1}\,K^{-1}}$
& meV
& meV
& $\mathrm{m}a_0^2$
& meV
& meV
& meV \\

\midrule
\multicolumn{13}{l}{\emph{Invariant models}} \\
\midrule

Cormorant
& 85
& 61
& 34
& 38
& 38
& 26
& 20
& 21
& 961
& 21
& 22
& 2.03 \\

NMP
& 92
& 69
& 43
& 38
& 30
& 40
& 19
& 17
& 180
& 20
& 20
& 1.50 \\

DimeNet++$\dagger$
& 44
& 32.6
& 24.6
& 19.5
& 29.7
& 23
& 7.56
& 6.53
& 331
& 6.28
& 6.32
& 1.21 \\

ComENet$\dagger$
& 45
& 32.4
& 23.1
& 19.8
& 24.5
& 22
& 7.98
& 6.86
& 259
& 6.82
& 6.69
& 1.20 \\

SphereNet$\dagger$
& 46
& 31.1
& 22.8
& 18.9
& 24.5
& 22
& 7.78
& 6.33
& 268
& 6.36
& 6.26
& 1.12 \\

\midrule
\multicolumn{13}{l}{\emph{Scalarization-based models}} \\
\midrule

ClofNet
& 63
& 53
& 33
& 25
& 40
& 27
& 9
& 9
& 610
& 9
& 8
& 1.23 \\

EGNN
& 71
& 48
& 29
& 25
& 29
& 31
& 12
& 12
& 106
& 12
& 11
& 1.55 \\

PaiNN$\dagger$
& 45
& 45.7
& 27.6
& 20.4
& 12.0
& 24
& 7.35
& 5.98
& 66
& 5.83
& 5.85
& 1.28 \\

LEFTNet
& 48
& 40
& 24
& 18
& 12
& 23
& 7
& 6
& 109
& 7
& 6
& 1.33 \\

EQGAT
& 53
& 32
& 20
& 16
& 11
& 24
& 23
& 24
& 382
& 25
& 25
& 2.00 \\

ET
& 59
& 36.1
& 20.3
& 17.5
& 11
& 26
& 7.62
& 6.16
& 33
& 6.38
& 6.15
& 1.84 \\

Geoformer
& 40
& 33.8
& 18.4
& 15.4
& 10
& 22
& 6.13
& 4.39
& 28
& 4.41
& 4.43
& 1.28 \\

SaVeNet-B$\dagger$
& 39
& 24.8
& 18.4
& 16.3
& 9.3
& 23
& 6.64
& 5.43
& 58
& 5.48
& 5.43
& 1.18 \\

\midrule
\multicolumn{13}{l}{\emph{Equivariant Sheaf Neural Networks}} \\
\midrule

\textbf{ESNN-Id}
& 63.08
& 65.35
& 43.13
& 28.52
& 58.81
& 37.83
& 15.76
& 18.71
& 749.44
& 10.67
& 10.54
& 1.54 \\

\textbf{ESNN-Diag}
& 62.16
& 43.69
& \textbf{20.29}
& 21.43
& 17.15
& \textbf{30.57}
& \textbf{11.48}
& \textbf{12.09}
& 110.88
& 11.77
& 13.57
& 1.62 \\

\textbf{ESNN-Ortho}
& 79.42
& 43.35
& 25.10
& 23.17
& 21.77
& 36.50
& 17.76
& 26.07
& 323.52
& 18.59
& 25.25
& 1.94 \\

\textbf{ESNN-RadTan}
& \textbf{55.90}
& \textbf{39.01}
& 25.16
& \textbf{19.17}
& \textbf{13.99}
& 31.57
& 14.77
& 13.86
& \textbf{108.16}
& \textbf{10.63}
& \textbf{10.34}
& \textbf{1.45} \\

\bottomrule
\end{tabular}%
}
\end{table*}
